Challenges and Opportunities in Approximate Bayesian Deep Learning for Intelligent IoT Systems

Approximate Bayesian deep learning methods hold significant promise for addressing several issues that occur when deploying deep learning components in intelligent systems, including mitigating the occurrence of over-confident errors and providing enhanced robustness to out of distribution examples. However, the computational requirements of existing approximate Bayesian inference methods can make them ill-suited for deployment in intelligent IoT systems that include lower-powered edge devices. In this paper, we present a range of approximate Bayesian inference methods for supervised deep learning and highlight the challenges and opportunities when applying these methods on current edge hardware. We highlight several potential solutions to decreasing model storage requirements and improving computational scalability, including model pruning and distillation methods.

==> evaluation.tex <==
\section{Evaluation Considerations}
\label{sec:evaluation_considerations}
While discussing the motivation for BNNs against traditional point-estimated neural networks earlier in the paper, we highlighted that the unique aspect about BNNs is that they capture the uncertainty in parameter estimation while making predictions. As a result, we cannot only rely on traditional supervised learning metrics, which mainly focus around accuracy. \emph{URSABench} \cite{Vadera2020URSABenchCB} provides a comprehensive evaluation framework for approximate inference techniques. We leverage that framework and provide four facets of evaluation: predictive performance, uncertainty quantification, robustness, and scalability. These four aspects are described below in brief. 

\textbf{Predictive Performance:} Predictive performance, quite simply, looks at how well can model predict on held-out test data by probabilistic thresholding. In the classification setting, evaluation measures that only require that the true label $y$ be correctly predicted provide the coarsest measures of the predictive performance. Such measures include accuracy, precision, recall, and F1 score. 

\textbf {Uncertainty Quantification:} In contrast to the assessment of predictive performance, we also need to assess how well our Bayesian methods can we quantify uncertainty in the probabilistic setting. A number of helpful metrics here include log likelihood and expected calibration error (ECE), and brier score.  Aside from these metrics, an additional useful task for in-domain uncertainty quantification is misclassification detection.

Predictive log likelihood can provide more insight into the model confidence while making predictions, as it is sensitive to the predictive probability of $p(y| \mathbf{x}, \mathcal{D}_{tr},\theta^0)$. Overconfident errors and under-confident accurate predictions both affect the log-likelihood adversely. For perfect log likelihood, we would want the predictive probably for the ground truth class to be 1. 

Calibration is also an important property of predictive models, and recent evaluations of deep learning methods have shown that their calibration properties can be quite poor \cite{guo2017calibration}. In the binary classification case, a classifier is said to be perfectly calibrated if exactly $p$ percent of instances are predicted to be positive with $p$ percent probability. The degree of calibration of a binary classifier can be quantified using the expected calibration error (ECE) \cite{guo2017calibration}. In the case of multi-class classification, a one-vs-all formulation of calibration error can be used. The Brier score provides an alternate measure of calibration \cite{brier1950verification} that can be interpreted as combining the aspects of calibration and accuracy. 

Finally, misclassification detection  \cite{Hendrycks2017ABF} performance is also helpful in assessing how useful an indicator are uncertainty metrics for misclassified examples.

\textbf{Robustness:} Another key property of models and inference methods is their robustness. As we highlighted earlier, in practical scenarios our intelligent systems can receive inputs that are out of the domain that they were trained on, or they can also receive adversarial manipulated images that are designed to fool them. The metrics that we've looked at so far are typically computed on a test data set $\mathcal{D}_{te}$ that is assumed to be sampled from the same distribution as the training data set $\mathcal{D}_{tr}$. Out-of-distribution (OOD) detection tasks instead assess the ability of methods to detect examples from a set $\mathcal{D}_{ood}$ drawn from a different distribution than $\mathcal{D}_{tr}$ \cite{Ovadia2019can}. Under the OOD task, our aim is to evaluate how well of an indicator is the model confidence or the different quantities of uncertainty that we saw in section \ref{sec:bnn_background} are in determining if the input is out of distribution. The ability of methods to resist adversarial input perturbations as measured by the success rate of different adversarial attacks is also an important property \cite{Goodfellow2015ICLR, madry2018towards,Carlini2017}. We note that in the Bayesian supervised learning context, these attack methods require access to the posterior predictive distribution function and in many cases its gradients \cite{Vadera2020AssessingTA}.

\textbf{Scalability:} Scalability is of paramount interest, as we aim to perform approximate Bayesian inference at the edge. The storage cost can be estimated via the number of parameters and the size of stored models (if variable bit depth is considered). The run-time of methods can be assessed in different ways, including wall clock time as well as more fundamental metrics such as the number of FLOPS or multiply-accumulate operations (MACs). The performance-scalability tradeoff must be assessed while choosing between approximate inference techniques for more efficient edge deployments.

==> opportunities_challenges.tex <==
\section{Architectural Approaches to Improving \\the Scalability of Bayesian Deep Learning}
\label{sec:opportunities_challenges}
The previous sections of this paper have discusses challenges and opportunities with potential modeling and algorithmic approaches to improving the computational scalability of approximate Bayesian deep learning. In this section, we consider architectural approaches to improving scalability, with the focus 

Throughout this paper, we touched upon different approximate Bayesian inference algorithms, the inherent scalability issues with them, and how one might look at scaling them for low-resource edge environments.
%We also provided a set of evaluation consideration that to assess these different methods. Now, as we combine the different techniques mentioned in this paper, a new set of challenges and opportunities arise from a practitioner's perspective. 

The first challenge is associated with optimizing the model deployment for the specific edge hardware. There's a wide range of edge devices with different capabilities in terms of processing speed, storage, power requirements, and support for quantization-enabled inference. Prominent examples of edge hardware include NVIDIA Jetson Nano, Jetson Xavier, and GAP8 among others. More crucially, each edge device requires a unique optimization of model inference to achieve the lowest possible latency for the particular device. One such optimization SDK is TensorRT \cite{tensorrt} for NVIDIA Jetson devices. TensorRT takes as input the model, along with the model parameters, and provides an optimized version of it. Now, a caveat here is that TensorRT cannot directly take the model checkpoints saved from the deep learning library. Instead, it requires the model representation in terms of a static computation graph, which can be built using Open Neural Network Exchange (ONNX) \cite{bai2019}. An issue here is that while generating the static computation graph, ONNX gets rid of all the stochastic operations (such as dropout, batch normalization, etc.), and thus adds additional difficulties for implementing MC Dropout. A workaround here would be to implement last-layer MC dropout, where we introduce dropout only before the final layer of our model. Then, we can emulate MC Dropout by generating multiple parameter matrices with the final layer (which is usually a feed-forward linear layer), each with a set of weight vectors masked at random. This also leads to additional storage requirement, as we now need to store multiple copies for the final layer. Of course, this can be extended to other approximate inference techniques as well, where we perform Bayesian inference only on a set of final layers rather than the entire model.

The second challenge, closely associated with the first one, is the pre-processing time required for deployment. The process of converting a trained model to an optimized version for edge deployment can sometimes be time-consuming. Now, for doing this pre-processing step for every model in the Bayesian ensemble scales the time requirement linearly. This can be detrimental, especially when our application involves having to regularly update our Bayesian ensemble and deploy it back quickly. This pre-processing overhead, along with additional storage-computation benefits, makes distilled posterior representations slightly more favorable as compared to the corresponding Bayesian ensembles.

The third challenge is with respect to performing inference through multiple models in the Bayesian ensemble for CUDA devices. For computing the monte carlo approximation of posterior predictive distribution, we need to run our inputs by every member of the ensemble, which scales linearly with the size of the ensemble. Recall that for point-estimated neural network models, we can perform inference on multiple inputs by mini-batching the inputs for a given model, which is able to leverage parallelism in the computing hardware and the runtime doesn't scale linearly with the size of the mini-batch. Now, for Bayesian ensembles, at inference time we have a single input, but multiple models. To leverage the parallelism offered by CUDA devices, we can generate a meta-model that takes a single input, and runs it through each of the members of the ensemble and averages the output. When we generate the forward computation graph of the meta-model through ONNX, we will see that this will be equivalent to running the input through different members of the ensemble simultaneously, and will be able to realize the speedup at the time of inference.

Finally, the myriad of posterior compression methods (and their potential combinations) that we discussed in this paper warrant a fair and comprehensive comparison against each other. The individual papers that present these methods have their own evaluation strategy, and do not compare against all other existing methods. For instance, in the current literature, we do not have a benchmark that compares unstructured pruning methods against structured pruning methods. More importantly, we also need these comparisons in the context of Bayesian ensembles as that can shift performance trends from point-estimated neural networks. Future benchmarks should ensure that the evaluation considerations proposed in this paper are taken into account to generate a robust set of comparisons.
